Where Responsible AI meets Reality: Practitioner Perspectives on Enablers for shifting Organizational Practices

Large and ever-evolving technology companies continue to invest more time and resources to incorporate responsible Artificial Intelligence (AI) into production-ready systems to increase algorithmic accountability. This paper examines and seeks to offer a framework for analyzing how organizational culture and structure impact the effectiveness of responsible AI initiatives in practice. We present the results of semi-structured qualitative interviews with practitioners working in industry, investigating common challenges, ethical tensions, and effective enablers for responsible AI initiatives. Focusing on major companies developing or utilizing AI, we have mapped what organizational structures currently support or hinder responsible AI initiatives, what aspirational future processes and structures would best enable effective initiatives, and what key elements comprise the transition from current work practices to the aspirational future.

==> workshop_scenarios.tex <==
\section{Scenarios}
\subsection{OKLinger}

A company called OKLinger is developing a dating service which uses ML systems to make recommendations for a user’s entire dating life to maximize a user’s “happiness score” - from who to ask out and where to go to dinner to whether to go home together, and even when to end the relationship. Work on fairness, accountability, and transparency of their algorithmic systems is not very common, but a few team-members have been bringing it up again and again during meetings. OKLinger’s leadership has not spoken about this topic internally or externally. Some employees have expressed their concerns that there's a lack of understanding about the potential issues, the impacts of the unintended consequences of their technology, as well as latent uncertainty about the alignment between OKLinger’s products and its employees’ broader societal values and beliefs.

\subsection{BreatheResponsibly}
A company called BreatheResponsibly develops a carbon offsets platform which makes recommendations on where to offset carbon. Carbon offsets compensate for your emissions by canceling out greenhouse gas emissions somewhere else in the world. The money you pay to buy offsets supports programs designed to reduce emissions. Work on fairness, accountability, and transparency of their recommendation engine is not very common, however a few team-members have been bringing it up again and again during meetings. BreatheResponsibly's leadership has not spoken about this topic internally or externally. Some employees have expressed their concerns that there's a lack of understanding about the potential issues, the impacts of the unintended consequences of their technology, as well as latent uncertainty about the alignment between BreatheResponsibly's products and its employees’ broader societal values and beliefs. 
\subsection{FeetMirror}
A company called FeetMirror is building a social media platform to engage youth in South Africa. They have an advertisement-based business model and are promoting western brands using ML to target advertisements to their users. Work on fairness, accountability, and transparency of their algorithmic systems is not very common, but a few team members have been bringing it up again and again during meetings. FeetMirror's leadership has not spoken about this topic internally or externally. Some employees have expressed their concerns that there's a lack of understanding about the potential issues, the impacts of the unintended consequences of their technology, as well as latent uncertainty about the alignment between FeetMirror's products and its employees’ broader societal values and beliefs.  

\subsection{EmptyFrisk}
A company called EmptyFrisk is developing a risk assessment tool - a predictive model to assess the risk that a defendant fails to appear in court to aid in decision-making at various stages of the criminal justice pipeline. The output of the model is a risk score number. This risk assessment tool is used to determine whether defendants should be released pretrial and whether bail should be required. In most jurisdictions, EmptyFrisk’s risk scores are presented to a judge as a recommendation. Work on fairness, accountability, and transparency of EmptyFrisk’s algorithmic systems is not very common, but a few team-members have been bringing it up again and again during meetings.  EmptyFrisk's leadership has not spoken about this topic internally or externally. Some employees have expressed their concerns that there's a lack of understanding about the potential issues, the impacts of the unintended consequences of their technology, as well as latent uncertainty about the alignment between EmptyFrisk’s products and its employees’ broader societal values and beliefs.  
